Object Segmentation from Open-Vocabulary Manipulation Instructions Based on Optimal Transport Polygon Matching with Multimodal Foundation Models

We consider the task of generating segmentation masks for the target object from an object manipulation instruction, which allows users to give open vocabulary instructions to domestic service robots. Conventional segmentation generation approaches often fail to account for objects outside the camera's field of view and cases in which the order of vertices differs but still represents the same polygon, which leads to erroneous mask generation. In this study, we propose a novel method that generates segmentation masks from open vocabulary instructions. We implement a novel loss function using optimal transport to prevent significant loss where the order of vertices differs but still represents the same polygon. To evaluate our approach, we constructed a new dataset based on the REVERIE dataset and Matterport3D dataset. The results demonstrated the effectiveness of the proposed method compared with existing mask generation methods. Remarkably, our best model achieved a +16.32% improvement on the dataset compared with a representative polygon-based method.

==> tab/confusion_matrix_alfred-fc.tex <==
\begin{table}[t]
    \normalsize
    \caption{\small Confusion matrix on the ALFRED-fc dataset}
    \label{tab:confusion_matrix_alfred-fc}
    \centering
    \begin{tabular}{|c|c||cc|}
        \hline
        \multicolumn{2}{|c||}{} & \multicolumn{2}{c|}{Predicted Label} \\
        \cline{3-4}
        \multicolumn{2}{|c||}{} & \multicolumn{1}{c}{Positive} & \multicolumn{1}{c|}{Negative} \\
        \hline
        \hline
        True Label & Positive & 453 & 233 \\
        % \cline{2-4}
        & Negative & 24  & 662 \\
        \hline
    \end{tabular}
\end{table}
% TODO: 混同行列の書き方がこれで望ましいか
% スペースの都合で文にした


==> tab/error.tex <==
% \begin{table}[t]
%     \caption{\small Categories of failure cases on the ALFRED-fc dataset}
%     \label{tab:error}
%     \centering
%     \scalebox{0.9}{
%         \begin{tabular}{clcc}
%             \hline
%             \begin{tabular}{c}
%                 Error ID
%             \end{tabular} &
%             \begin{tabular}{l}
%                 Description
%             \end{tabular} &
%             \begin{tabular}{c}
%                 Target Mode
%             \end{tabular} &
%             \begin{tabular}{c}
%                 Destination Mode
%             \end{tabular} \\
%             \hline\hline
%             SC &
%             \begin{tabular}{l}
%                 % Serious Comprehension error
%                 xxx
%             \end{tabular} &
%             34 & 25 \\
%             SOF &
%             \begin{tabular}{l}
%                 % Similar Object or Furniture
%                 xxx
%             \end{tabular} &
%             8 & 7 \\
%             SR &
%             \begin{tabular}{l}
%                 % Small Region
%                 xxx
%             \end{tabular} &
%             7 & 0 \\
%             IVI &
%             \begin{tabular}{l}
%                 % Insufficient Visual Information
%                 xxx
%             \end{tabular} &
%             0 & 15 \\
%             II &
%             \begin{tabular}{l}
%                 % Incomplete Instruction
%                 xxx
%             \end{tabular} &
%             0 & 1 \\
%             IL &
%             \begin{tabular}{l}
%                 % Incorrect Label
%                 xxx
%             \end{tabular} &
%             1 & 2 \\
%             \hline\hline
%             Total &
%             \begin{tabular}{l}
%                 -
%             \end{tabular} &
%             50 & 50 \\
%             \hline
%         \end{tabular}
%     }
% \end{table}

\begin{table}[t]
    \caption{\small Categories of failure cases on the ALFRED-fc dataset}
    \label{tab:error}
    % \normalsize
    \centering
    \begin{tabular}{ccc}
        \hline
        \begin{tabular}{c}
            Error ID
        \end{tabular} &
        \begin{tabular}{c}
            Target Mode
        \end{tabular} &
        \begin{tabular}{c}
            Destination Mode
        \end{tabular} \\
        \hline\hline
        SC &
        34 & 25 \\
        SOF &
        8 & 7 \\
        % SR &
        TR &
        7 & 0 \\
        IVI &
        0 & 15 \\
        % II &
        % 0 & 1 \\
        % IL &
        % 1 & 2 \\
        Others &
        1 & 3 \\
        \hline\hline
        Total &
        50 & 50 \\
        \hline
    \end{tabular}
    \vspace{-5mm}
\end{table}
% TODO: 見出し行を2段にする↓のとどちらが良い？
% TODO: 2段にしてdescriptionを復活？
% \begin{table}[t]
%     \caption{\small Categories of failure cases on the ALFRED-fc dataset}
%     \label{tab:error}
%     \normalsize
%     \centering
%     \begin{tabular}{ccc}
%         \hline
%         \begin{tabular}{c}
%             Error\\
%             ID
%         \end{tabular} &
%         \begin{tabular}{c}
%             Target\\
%             Mode
%         \end{tabular} &
%         \begin{tabular}{c}
%             Destination\\
%             Mode
%         \end{tabular} \\
%         \hline\hline
%         SC &
%         34 & 25 \\
%         SOF &
%         8 & 7 \\
%         TR &
%         7 & 0 \\
%         IVI &
%         0 & 15 \\
%         II &
%         0 & 1 \\
%         IL &
%         1 & 2 \\
%         \hline\hline
%         Total &
%         50 & 50 \\
%         \hline
%     \end{tabular}
% \end{table}


==> tab/params.tex <==
\begin{table}[t]
    \normalsize
    \centering
    \caption{\small Parameter settings of SHeFU}
    \label{tab:parameters}
    \begin{tabular}{|c|l|}
        \hline
        Optimizer & Adam\\ & ($\beta_1=0.9$, $\beta_2=0.999$)\\
        \hline
        Learning Rate & $8\times10^{-5}$\\
        \hline
        Step & $20000$\\
        \hline
        Batch Size & $8$\\
        \hline
        Dropout & $0.1$\\
        \hline
        Task Weights & $\lambda_\mathrm{targ}=1.0$, $\lambda_\mathrm{dest}=1.0$\\
        \hline
        \end{tabular}
\end{table}
% 余白の都合で文にする


==> tab/quantitative_action.tex <==
\begin{table}[t]
    % \normalsize
    % \caption{\small Task success rates in the physical experiment}
    \caption{\small Task success rates in the physical experiments}
    \label{tab:quantitative_action}
    \centering
    \vspace{-1mm}
    \begin{tabular}{lcc}
        \hline
        % Task & $\frac{N_\mathrm{success}}{N_\mathrm{attempts}}$ & SR [\%]\\
        % Task & $N_\mathrm{success} / N_\mathrm{attempts}$ & SR [\%]\\
        Task & $N_\mathrm{s} / N_\mathrm{a}$ & SR [\%]\\
        \hline\hline
        Grasping & $60$ / $63$ & $95$\\
        Placing & $56$ / $60$ & $93$\\
        \hline
    \end{tabular}
    % \vspace{-5mm}
    \vspace{-5.45mm}
\end{table}


==> tab/quantitative_language.tex <==
\begin{table}
    \normalsize
    % \caption{\small Quantitative results on the ALFRED-fc dataset and the real-world environment}
    \caption{\small Language comprehension accuracy on the \\ALFRED-fc dataset and the real-world environment}
    \label{tab:quantitative_language}
    \centering
    \scalebox{.95}{
        \begin{tabular}{m{0.5em}lcc}
            \hline
            % & & \multicolumn{2}{c}{Accuracy [\%]}\\
            % & Method & ALFRED-fc & Real\\
            [\%] & \;Method & ALFRED-fc & Real\\
            \hline\hline
            % (i) & \;Baseline (extended TdU~\cite{ishikawa2021target}) & $79.4 \pm 2.76$ & $52.0$\\
            (i) & \;Baseline (extended TDU~\cite{ishikawa2021target}) & $79.4 \pm 2.76$ & $52.0$\\
            % (ii) & \;Ours (W/o xxx) & $78.4 \pm 2.05$ & -\\
            % (ii) & \;Ours (W/o Switching head) & $78.4 \pm 2.05$ & -\\
            (ii) & \;Ours (W/o Switching Head) & $78.4 \pm 2.05$ & -\\
            % (iii) & \;Ours (W/o xxx) & $76.9 \pm 2.91$ & -\\
            % (iii) & \;Ours (W/o Switching tail) & $76.9 \pm 2.91$ & -\\
            (iii) & \;Ours (W/o Switching Tail) & $76.9 \pm 2.91$ & -\\
            (iv) & \;Ours (SHeFU) & $\mathbf{83.1 \pm 2.00}$ & $\mathbf{55.9}$\\
            \hline
        \end{tabular}
    }
    % \vspace{-5mm}
    % 大事な表なので余白多め
    \vspace{-4mm}
\end{table}

